LLMDFA: Analyzing Dataflow in Code with Large Language Models

Dataflow analysis is a fundamental code analysis technique that identifies dependencies between program values. Traditional approaches typically necessitate successful compilation and expert customization, hindering their applicability and usability for analyzing uncompilable programs with evolving analysis needs in real-world scenarios. This paper presents LLMDFA, an LLM-powered compilation-free and customizable dataflow analysis framework. To address hallucinations for reliable results, we decompose the problem into several subtasks and introduce a series of novel strategies. Specifically, we leverage LLMs to synthesize code that outsources delicate reasoning to external expert tools, such as using a parsing library to extract program values of interest and invoking an automated theorem prover to validate path feasibility. Additionally, we adopt a few-shot chain-of-thought prompting to summarize dataflow facts in individual functions, aligning the LLMs with the program semantics of small code snippets to mitigate hallucinations. We evaluate LLMDFA on synthetic programs to detect three representative types of bugs and on real-world Android applications for customized bug detection. On average, LLMDFA achieves 87.10% precision and 80.77% recall, surpassing existing techniques with F1 score improvements of up to 0.35. We have open-sourced LLMDFA at https://github.com/chengpeng-wang/LLMDFA.

==> alg.tex <==
\begin{algorithm}[t]
	\caption{Data Flow Analysis as an AI Agent}
	\label{alg:policy}
	\begin{algorithmic}
		\STATE {\bfseries Input:} Environment $\text{Env} = (P, G)$
		\STATE Initialize $\text{Mem} = (\emptyset, \emptyset, \emptyset)$.
		\FOR{$f \in P$}
		\STATE $(\text{Env}, \text{Mem}) = \alpha_s[f](\alpha_e[f](\text{Env}, \text{Mem}))$
		%\STATE $(\text{Env}, \text{Mem}) = \alpha_s[f](\text{Env}, \text{Mem})$
		\ENDFOR
		\FOR{$f \in P, \ g \in P$}
		\STATE $(\text{Env}, \text{Mem}) = \alpha_v[f, g](\text{Env}, \text{Mem})$
		\ENDFOR
		\STATE $(V_M, E_M, B_M) = \text{Mem}$
        \STATE \textbf{return} $B_M$
	\end{algorithmic}
\end{algorithm}

==> extractor_synthesis.tex <==
\subsubsection{Prompt in the action Extract: Synthesis Phase}

Please synthesize a tree-sitter parser in Python to extract sink from Java code sink from the AST of Java code.

The rules of the sink are as follows:

    - If there is an binary operation either division `/' or modulo `\%', then the second operand of the binary operation is sink.
    

Here's a list of examples of sink:

\textbf{Example 1:}

\mybox{
\textbf{int} x = 0;\\
\textbf{int} z = 1 + x;\\
\textbf{int} y = z / x;  //Sink: x
}

The corresponding AST of the above code is:
\mybox{
[local\_variable\_declaration] `\textbf{int} x = 0;'\\
...
}

\textbf{Example 2:}

\mybox{
\textbf{int} x = Integer.parseInt(input.trim());\\
\textbf{int} y = 1 \% x;   // Sink: x
}

The corresponding AST of the above code is:
\mybox{
...
}

\textbf{Example 3:}

\mybox{
\textbf{int} x = foo();\\
goo();\\
woo();\\
yoo();
}

The corresponding AST of the above code is:
\mybox{
...
}

\textbf{Example 4:}

\mybox{
\textbf{int} x = 2;\\
x = 1 + x;\\
x = 0;\\
\textbf{int} y = Integer.parseInt(input.trim());\\
x = 1 $\%$ y; //Sink: y
}

The corresponding AST of the above code is:
\mybox{
...
}


The AST tree presents the tree structure in which each line is a node in the tree and the indentation indicates the parent-child relationship.
Children of a node are printed in order, starting from index 0. The node is represented as `index [type] text', where index is the child index of current node in its parent node, type is the node type of the current node, and
text is the string text of the node.
            
Please synthesize the tree-sitter AST parser that considering the structure and node information in the above code examples,
based on the following skeleton of a tree-sitter AST parser. You should focus on filling the placeholders in the template
according to the instructions in the TODO comments.

\mybox{
\textbf{from} tree\_sitter \textbf{import} Node\\
\textbf{from} synthesis.utils \textbf{import} DFValue\\

\textbf{def} find\_sink(source\_code: str, root\_node: Node):\\
\hspace*{0.5cm}\# Extract sources from the given code.\\
\hspace*{0.5cm}\# TODO: fill the node type \_\_TYPE\_\_ here\\
\hspace*{0.5cm}nodes = find\_nodes\_by\_type(root\_node, \_\_TYPE\_\_)\\
\hspace*{0.5cm}sink\_nodes = []\\
\hspace*{0.5cm}\textbf{for}   node \textbf{in} nodes:\\
\hspace*{1cm}\# TODO: fill the condition \_\_COND\_\_ here\\
\hspace*{1cm}\textbf{if} \_\_COND\_\_:\\
\hspace*{1.5cm}sink\_nodes.append(node)\\

\hspace*{0.5cm}sinks = []\\
\hspace*{0.5cm}\textbf{def} extract\_sinks(n: Node):\\
\hspace*{1cm}sink\_values = []\\
\hspace*{1cm}\# TODO: Extract sinks from the given node.\\
\hspace*{1cm}\# Below are two useful utility functions:\\
\hspace*{1cm}\# - Utility function I: get\_argument\_list: \\
\hspace*{1cm}\#\# \ extract the arguments from a method\\
\hspace*{1cm}\# - Utility function II: get\_binexpr\_operands: \\
\hspace*{1cm}\#\# \ extract the operands from a binary \\
\hspace*{1cm}\#\# \ expression node\\
\hspace*{1cm}\# Each of the sink nodes should be a tuple\\
\hspace*{1cm}\#\# \ (line number, sink variable name,``sink").\\
\hspace*{1cm}\textbf{return}  sink\_values\\

\hspace*{0.5cm}\textbf{for}   node \textbf{in} sink\_nodes:\\
\hspace*{1cm}sinks.extend(extract\_sinks(node))\\
\hspace*{0.5cm}\textbf{return}  sinks
}

Please directly output code without any other description.
In the code, please output the `find\_dbz\_sink' function only.

    
We offer several utility functions to help you extract sources and sinks from the given code.
\begin{itemize}
    \item To get the line number of a node, use `get\_line\_number(source\_code: str, node: Node) $\rightarrow$ int'.

    \item To get the list of arguments from a function call, use `get\_argument\_list(node: Node) $\rightarrow$ list[Node]'.

    \item To get the list of operands from a binary expression, use `get\_binexpr\_operands(node: Node) $\rightarrow$ list[Node]'.

    \item To find a node with the given type in the children of one node recursively, use `find\_nodes\_by\_type(node: Node, child\_node\_type: str) $\rightarrow$ list[Node]'.
\end{itemize}

The `child\_node\_type' must be one of the node types in the tree-sitter AST.\\

In addition, here are some useful usage of AST nodes:\\
- To get the line number of a node, use `source\_code[: node.start\_byte].count(``$\backslash$n'') + 1'.\\
- To get the text of a node, use `source\_code[node.start\_byte: node.end\_byte]'.\\

    
In the following are some useful usage of AST trees:
Given the following code and AST tree:

\mybox{
\textbf{int} x = 0;
}

\mybox{
[local\_variable\_declaration] `\textbf{int} x = 0;'\\
...
}


The root node is of type `local\_variable\_declaration', and it has 3 children of the following type: `integral\_type', `variable\_declarator', and `;'.
In other to get all the children node of a type, say `decimal\_integer\_literal', you can use `find\_nodes\_by\_type(root\_node,``decimal\_integer\_literal")',
which returns a list of child nodes of type `decimal\_integer\_literal'. Such child nodes may or may not be direct children of the root node.

To get the text of a node, say the node with type `variable\_declarator', you can use `source\_code[node.start\_byte: node.end\_byte]'.
In this example, the text of `variable\_declarator' node is `x = 0'.

If the task is to find an identifier in the source code whose name is `x', you can use the following code:

\mybox{
cs = find\_nodes\_by\_type(root\_node, `identifier')\\
\textbf{for}   ch \textbf{in} cs:\\
\hspace*{0.5cm}\textbf{if} source\_code[ch.start\_byte: ch.end\_byte] == `x':\\
\hspace*{1cm}        \# do something
}

\subsubsection{Response in the action Extract: Synthesis Phase}

\mybox{
\textbf{from} tree\_sitter \textbf{import} Node\\
\textbf{from} synthesis.utils \textbf{import} DFValue\\

\textbf{def} find\_sink(source\_code: str, root\_node: Node):\\
\hspace*{0.5cm}\# Extract sources from the given code.\\
\hspace*{0.5cm}\# TODO: fill the node type \_\_TYPE\_\_ here\\
\hspace*{0.5cm}nodes = find\_nodes\_by\_type(root\_node,\\
\hspace*{4.5cm}`binary\_expression')\\
\hspace*{0.5cm}sink\_nodes = []\\
\hspace*{0.5cm}\textbf{for}   node \textbf{in} nodes:\\
\hspace*{1cm}\# TODO: fill the condition \_\_COND\_\_ here\\
\hspace*{1cm}\textbf{if} len(get\_binexpr\_operands(node)) == 2:\\
\hspace*{1.5cm}sink\_nodes.append(node)\\

\hspace*{0.5cm}sinks = []\\
\hspace*{0.5cm}\textbf{def} extract\_sinks(n: Node):\\
\hspace*{1cm}sink\_values = []\\
\hspace*{1cm}\# TODO: Extract sinks from the given node.\\
\hspace*{1cm}\# Below are two useful utility functions:\\
\hspace*{1cm}\# - Utility function I: get\_argument\_list: \\
\hspace*{1cm}\#\# \ extract the arguments from a method\\
\hspace*{1cm}\# - Utility function II: get\_binexpr\_operands: \\
\hspace*{1cm}\#\# \ extract the operands from a binary \\
\hspace*{1cm}\#\# \ expression node\\
\hspace*{1cm}\# Each of the sink nodes should be a tuple\\
\hspace*{1cm}\#\# \ (line number, sink variable name,``sink").\\
\hspace*{1cm}line = get\_line\_number(source\_code, n)\\
\hspace*{1cm}name = source\_code[n.start\_byte: n.end\_byte]\\
\hspace*{1cm}sink\_values.append((line, name, ``sink''))\\
\hspace*{1cm}\textbf{return}  sink\_values\\

\hspace*{0.5cm}\textbf{for}   node \textbf{in} sink\_nodes:\\
\hspace*{1cm}sinks.extend(extract\_sinks(node))\\
\hspace*{0.5cm}\textbf{return}  sinks
}

\subsubsection{Prompt in the action Extract: Fix Phase}

Given the following script:

\mybox{
\textbf{from} tree\_sitter \textbf{import} Node\\
\textbf{from} synthesis.utils \textbf{import} DFValue\\

\textbf{def} find\_sink(source\_code: str, root\_node: Node):\\
\hspace*{0.5cm}\# Extract sources from the given code.\\
\hspace*{0.5cm}\# TODO: fill the node type \_\_TYPE\_\_ here\\
\hspace*{0.5cm}nodes = find\_nodes\_by\_type(root\_node,\\
\hspace*{4.5cm}`binary\_expression')\\
\hspace*{0.5cm}sink\_nodes = []\\
\hspace*{0.5cm}\textbf{for}   node \textbf{in} nodes:\\
\hspace*{1cm}\# TODO: fill the condition \_\_COND\_\_ here\\
\hspace*{1cm}\textbf{if} len(get\_binexpr\_operands(node)) == 2:\\
\hspace*{1.5cm}sink\_nodes.append(node)\\

\hspace*{0.5cm}sinks = []\\
\hspace*{0.5cm}\textbf{def} extract\_sinks(n: Node):\\
\hspace*{1cm}sink\_values = []\\
\hspace*{1cm}\# TODO: Extract sinks from the given node.\\
\hspace*{1cm}\# Below are two useful utility functions:\\
\hspace*{1cm}\# - Utility function I: get\_argument\_list: \\
\hspace*{1cm}\#\# \ extract the arguments from a method\\
\hspace*{1cm}\# - Utility function II: get\_binexpr\_operands: \\
\hspace*{1cm}\#\# \ extract the operands from a binary \\
\hspace*{1cm}\#\# \ expression node\\
\hspace*{1cm}\# Each of the sink nodes should be a tuple\\
\hspace*{1cm}\#\# \ (line number, sink variable name,``sink").\\
\hspace*{1cm}line = get\_line\_number(source\_code, n)\\
\hspace*{1cm}name = source\_code[n.start\_byte: n.end\_byte]\\
\hspace*{1cm}sink\_values.append((line, name, ``sink''))\\
\hspace*{1cm}\textbf{return}  sink\_values\\

\hspace*{0.5cm}\textbf{for}   node \textbf{in} sink\_nodes:\\
\hspace*{1cm}sinks.extend(extract\_sinks(node))\\
\hspace*{0.5cm}\textbf{return}  sinks
}

\textbf{Feedback I:} The sinks in the following examples are missed by the synthesized parser:

\textbf{Missing Case 1:} The sink `x' at line 3 in the following code is missed:

\mybox{
\textbf{int} x = 0;\\
\textbf{int} z = 1 + x;\\
\textbf{int} y = z / x;  //Sink: x
}

The corresponding AST of the above code is:
\mybox{
[local\_variable\_declaration] `\textbf{int} x = 0;'\\
...
}

\textbf{Missing Case 2:} The sink `x' at line 2 in the following code is missed:

\mybox{
\textbf{int} x = Integer.parseInt(input.trim());\\
\textbf{int} y = 1 \% x;   // Sink: x
}

The corresponding AST of the above code is:
\mybox{
...
}

\textbf{Missing Case 3:} The sink `y' at line 5 in the following code is missed:

\mybox{
\textbf{int} x = 2;\\
x = 1 + x;\\
x = 0;\\
\textbf{int} y = Integer.parseInt(input.trim());\\
x = 1 $\%$ y; //Sink: y
}

The corresponding AST of the above code is:
\mybox{
...
}

To identify the above missing sinks, you may want to loosen the conditions in the parser to cover the above examples.

\textbf{Feedback II:} The sinks in following examples are wrongly extracted by the synthesized extractor:


\textbf{Misidentified Case 1:}
The sink `1 + x' at line 2 in the following code is not sink, but the parser identifies it.

\mybox{
\textbf{int} x = 0;\\
\textbf{int} z = 1 + x;\\
\textbf{int} y = z / x;  //Sink: x
}

The corresponding AST of the above code is:
\mybox{
[local\_variable\_declaration] `\textbf{int} x = 0;'\\
...
}

\textbf{Misidentified Case 2:}
The sink `z / x' at line 2 in the following code is not sink, but the parser identifies it.

\mybox{
\textbf{int} x = 0;\\
\textbf{int} z = 1 + x;\\
\textbf{int} y = z / x;  //Sink: x
}

The corresponding AST of the above code is:
\mybox{
[local\_variable\_declaration] `\textbf{int} x = 0;'\\
...
}

\textbf{Misidentified Case 3:}
The sink `1 $\%$ x' at line 2 in the following code is not sink, but the parser identifies it:

\mybox{
\textbf{int} x = Integer.parseInt(input.trim());\\
\textbf{int} y = 1 \% x;   // Sink: x
}

The corresponding AST of the above code is:
\mybox{
...
}

\textbf{Misidentified Case 4:}
The sink `1 + x` at line 2 in the following code is not sink, but the parser identifies it:

\mybox{
\textbf{int} x = 2;\\
x = 1 + x;\\
x = 0;\\
\textbf{int} y = Integer.parseInt(input.trim());\\
x = 1 $\%$ y; //Sink: y
}

The corresponding AST of the above code is:
\mybox{
...
}

\textbf{Misidentified Case 5:}
The sink `1 $\%$ y' at line 5 in the following code is not sink, but the parser identifies it:

\mybox{
\textbf{int} x = 2;\\
x = 1 + x;\\
x = 0;\\
\textbf{int} y = Integer.parseInt(input.trim());\\
x = 1 $\%$ y; //Sink: y
}

The corresponding AST of the above code is:
\mybox{
...
}

You may want to combine multiple conditions in the parser to avoid the above examples.

Please re-synthesize a tree-sitter parser in Python to extract sink from Java code sink from the AST of Java code.

The rules of the sink are as follows:

    - If there is an binary operation either division `/' or modulo `\%', then the second operand of the binary operation is sink.

The AST tree presents the tree structure in which each line is a node in the tree and the indentation indicates the parent-child relationship.
Children of a node are printed in order, starting from index 0. The node is represented as `index [type] text', where index is the child index of current node in its parent node, type is the node type of the current node, and
text is the string text of the node.
            
Please synthesize the tree-sitter AST parser that considering the structure and node information in the above code examples,
based on the following skeleton of a tree-sitter AST parser. You should focus on filling the placeholders in the template
according to the instructions in the TODO comments.

\mybox{
\textbf{from} tree\_sitter \textbf{import} Node\\
\textbf{from} synthesis.utils \textbf{import} DFValue\\

\textbf{def} find\_sink(source\_code: str, root\_node: Node):\\
\hspace*{0.5cm}\# Extract sources from the given code.\\
\hspace*{0.5cm}\# TODO: fill the node type \_\_TYPE\_\_ here\\
\hspace*{0.5cm}nodes = find\_nodes\_by\_type(root\_node, \_\_TYPE\_\_)\\
\hspace*{0.5cm}sink\_nodes = []\\
\hspace*{0.5cm}\textbf{for}   node \textbf{in} nodes:\\
\hspace*{1cm}\# TODO: fill the condition \_\_COND\_\_ here\\
\hspace*{1cm}\textbf{if} \_\_COND\_\_:\\
\hspace*{1.5cm}sink\_nodes.append(node)\\

\hspace*{0.5cm}sinks = []\\
\hspace*{0.5cm}\textbf{def} extract\_sinks(n: Node):\\
\hspace*{1cm}sink\_values = []\\
\hspace*{1cm}\# TODO: Extract sinks from the given node.\\
\hspace*{1cm}\# Below are two useful utility functions:\\
\hspace*{1cm}\# - Utility function I: get\_argument\_list: \\
\hspace*{1cm}\#\# \ extract the arguments from a method\\
\hspace*{1cm}\# - Utility function II: get\_binexpr\_operands: \\
\hspace*{1cm}\#\# \ extract the operands from a binary \\
\hspace*{1cm}\#\# \ expression node\\
\hspace*{1cm}\# Each of the sink nodes should be a tuple\\
\hspace*{1cm}\#\# \ (line number, sink variable name,``sink").\\
\hspace*{1cm}\textbf{return}  sink\_values\\

\hspace*{0.5cm}\textbf{for}   node \textbf{in} sink\_nodes:\\
\hspace*{1cm}sinks.extend(extract\_sinks(node))\\
\hspace*{0.5cm}\textbf{return}  sinks
}

Please directly output code without any other description.
In the code, please output the `find\_dbz\_sink' function only.

    
We offer several utility functions to help you extract sources and sinks from the given code.
\begin{itemize}
    \item To get the line number of a node, use `get\_line\_number(source\_code: str, node: Node) $\rightarrow$ int'.

    \item To get the list of arguments from a function call, use `get\_argument\_list(node: Node) $\rightarrow$ list[Node]'.

    \item To get the list of operands from a binary expression, use `get\_binexpr\_operands(node: Node) $\rightarrow$ list[Node]'.

    \item To find a node with the given type in the children of one node recursively, use `find\_nodes\_by\_type(node: Node, child\_node\_type: str) $\rightarrow$ list[Node]'.
\end{itemize}

The `child\_node\_type' must be one of the node types in the tree-sitter AST.\\

In addition, here are some useful usage of AST nodes:\\
- To get the line number of a node, use `source\_code[: node.start\_byte].count(``$\backslash$n'') + 1'.\\
- To get the text of a node, use `source\_code[node.start\_byte: node.end\_byte]'.\\

    
In the following are some useful usage of AST trees:
Given the following code and AST tree:

\mybox{
\textbf{int} x = 0;
}

\mybox{
[local\_variable\_declaration] `\textbf{int} x = 0;'\\
...
}


The root node is of type `local\_variable\_declaration', and it has 3 children of the following type: `integral\_type', `variable\_declarator', and `;'.
In other to get all the children node of a type, say `decimal\_integer\_literal', you can use `find\_nodes\_by\_type(root\_node,``decimal\_integer\_literal")',
which returns a list of child nodes of type `decimal\_integer\_literal'. Such child nodes may or may not be direct children of the root node.

To get the text of a node, say the node with type `variable\_declarator', you can use `source\_code[node.start\_byte: node.end\_byte]'.
In this example, the text of `variable\_declarator' node is `x = 0'.

If the task is to find an identifier in the source code whose name is `x', you can use the following code:

\mybox{
cs = find\_nodes\_by\_type(root\_node, `identifier')\\
\textbf{for}   ch \textbf{in} cs:\\
\hspace*{0.5cm}\textbf{if} source\_code[ch.start\_byte: ch.end\_byte] == `x':\\
\hspace*{1cm}        \# do something
}

\subsubsection{Response in the action Extract: Fix Phase}

\mybox{
\textbf{from} tree\_sitter \textbf{import} Node\\
\textbf{from} synthesis.utils \textbf{import} DFValue\\

\textbf{def} find\_sink(source\_code: str, root\_node: Node):\\
\hspace*{0.5cm}\# Extract sources from the given code.\\
\hspace*{0.5cm}\# TODO: fill the node type \_\_TYPE\_\_ here\\
\hspace*{0.5cm}nodes = find\_nodes\_by\_type(root\_node,\\
\hspace*{4.5cm}`binary\_expression')\\
\hspace*{0.5cm}sink\_nodes = []\\
\hspace*{0.5cm}\textbf{for}   node \textbf{in} nodes:\\
\hspace*{1cm}\# TODO: fill the condition \_\_COND\_\_ here\\
\hspace*{1cm}text = source\_code[node.start\_byte:node.end\_byte]\\
\hspace*{1cm}\textbf{if} `/' \textbf{in} text \textbf{or} `$\%$; \textbf{in} text:\\
\hspace*{1.5cm}sink\_nodes.append(node)\\

\hspace*{0.5cm}sinks = []\\
\hspace*{0.5cm}\textbf{def} extract\_sinks(n: Node):\\
\hspace*{1cm}sink\_values = []\\
\hspace*{1cm}\# TODO: Extract sinks from the given node.\\
\hspace*{1cm}\# Below are two useful utility functions:\\
\hspace*{1cm}\# - Utility function I: get\_argument\_list: \\
\hspace*{1cm}\#\# \ extract the arguments from a method\\
\hspace*{1cm}\# - Utility function II: get\_binexpr\_operands: \\
\hspace*{1cm}\#\# \ extract the operands from a binary \\
\hspace*{1cm}\#\# \ expression node\\
\hspace*{1cm}\# Each of the sink nodes should be a tuple\\
\hspace*{1cm}\#\# \ (line number, sink variable name,``sink").\\
\hspace*{1cm}operands = get\_binexpr\_operands(node)\\
\hspace*{1cm}\textbf{if} len(operands) == 2:\\
\hspace*{1.5cm}sink\_node = operands[1]\\
\hspace*{1.5cm}line = get\_line\_number(source\_code, n)\\
\hspace*{1.5cm}m = source\_code[n.start\_byte: n.end\_byte]\\
\hspace*{1cm}sink\_values.append((line, m, ``sink''))\\
\hspace*{1cm}\textbf{return}  sink\_values\\

\hspace*{0.5cm}\textbf{for}   node \textbf{in} sink\_nodes:\\
\hspace*{1cm}sinks.extend(extract\_sinks(node))\\
\hspace*{0.5cm}\textbf{return}  sinks
}
